Attention, Please! Revisiting Attentive Probing Through the Lens of Efficiency

As fine-tuning becomes impractical at scale, probing is emerging as the preferred evaluation protocol. However, standard linear probing can understate the capability of models whose pre-training optimizes local representations rather than an explicit global representation. This motivates attentive probing, an alternative that uses attention to selectively aggregate patch-level features. Despite growing adoption, attentive probing is still underexplored: existing approaches are often over-parameterized and computationally inefficient. In this work, we revisit attentive probing through the lens of the accuracy vs. parameter-efficiency trade-off. We present the first comprehensive study of existing methods, analyzing their design choices and benchmarking their performance. Building on these insights, we propose efficient probing (EP), a lightweight yet effective multi-query cross-attention mechanism that eliminates redundant projections and reduces the number of trainable parameters. Across multiple benchmarks and pre-training paradigms, EP consistently outperforms linear probing and previous attentive probing methods, and remains effective when combined with parameter-efficient fine-tuning. Beyond evaluation, our analysis uncovers emerging properties of EP, including complementary attention maps, which open new directions for leveraging probing beyond protocol design. Project page: https://vrg.fel.cvut.cz/ep/.

==> plots/heatmaps.tex <==
%------------------------------------------------------------------------------
\begin{figure*}[ht]
  \centering
  % First row: Single-head variants
  \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/heatmaps/single_no_Wk.pdf}
    \caption{Single-head, $W_K$ fixed to identity.}
    \label{fig:single_no_Wk}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/heatmaps/single_with_Wk.pdf}
    \caption{Single-head with $W_K$.}
    \label{fig:single_with_Wk}
  \end{subfigure}
  % Second row: Multi-head variants
  \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/heatmaps/multi_no_Wk.pdf}
    \caption{Multi-head, $W_K$ fixed to identity.}
    \label{fig:multi_no_Wk}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/heatmaps/multi_with_Wk.pdf}
    \caption{Multi-head with $W_K$.}
    \label{fig:multi_with_Wk}
  \end{subfigure}

  \caption{\emph{Impact of $W_K$ in single-head (a, b) \vs multi-head attention (c, d).} In single-head attention, the distributions are nearly identical. In multi-head attention, the presence of $W_K$ alters the attention patterns.}
  \label{fig:heatmaps}
\end{figure*}
%------------------------------------------------------------------------------

==> tab/imagenet_val_extended_comparisons_with_pub.tex <==
    \begin{tabular}{c|lccc|c|cc|cc|c|cc}
        \toprule
         & \textsc{Method} & \textsc{Pub} & \textsc{Arch} & \textsc{Pre-training} & k-NN  & LP & \textsc{\# Par.} & EP & \textsc{\# Par.} & \textsc{Gain} & FT & \textsc{\# Par.} \\
        \midrule
        \multirow{6}{*}{\rotatebox{90}{MIM}} 
        & \multirow{3}{*}{MAE~\cite{mae}}     & \multirow{3}{*}{CVPR22} & ViT-S/16 & \multirow{3}{*}{IN-1K} & 26.7 & 47.4 & 0.4M & 64.6 & 0.5M & \textcolor{ForestGreen}{+17.2} & 80.6$^{\dagger}$ & \\
        & &  & ViT-B/16 &  & 46.1 & 67.7 & 0.8M & 75.6 & 1.4M & \textcolor{ForestGreen}{+7.9} & 83.6 & \\
        & &  & ViT-L/16 &  & 58.2 & 76.0 & 1.0M & 79.3 & 2.1M & \textcolor{ForestGreen}{+3.3} & 85.9 & \\
        \cline{2-13} \\ [-4pt]
        & BEiTv2~\cite{beitv2}  & arXiv22 & ViT-B/16 & IN‑1K & 74.8 & 79.0 & 0.8M & 81.7 & 1.4M & \textcolor{ForestGreen}{+2.7} & 85.0 & \\
        & SimMIM~\cite{simMIM}  & CVPR22 & ViT-B/16 & IN‑1K & 15.1 & 51.5 & 0.8M & 65.1 & 1.4M & \textcolor{ForestGreen}{+13.6} & 83.8 &  \\
        & CAPI~\cite{capi}    & TMLR25 & ViT-L/14 & IN‑1K & 76.7  & 81.5  & 1.0M & 83.6 & 2.1M & \textcolor{ForestGreen}{+2.1} & \textcolor{red}{$\times$} & \\
        \midrule
        \multirow{2}{*}{\rotatebox{90}{JEA}} & BYOL~\cite{byol}    & NeurIPS20 & RN-50 & IN‑1K & 64.8  & 74.3 & 2.0M & 75.1 & 6.3M & \textcolor{ForestGreen}{+0.8} & 77.7 &  \\
        & DINO~\cite{caron2021emerging}    & ICCV21 & ViT-B/16 & IN‑1K & 76.1  & 77.3 & 0.8M & 77.8 & 1.4M & \textcolor{ForestGreen}{+0.5} & 82.8 &  \\
        \midrule
        \multirow{7}{*}{\rotatebox{90}{HYBRID}} & iBOT~\cite{ibot}    & ICLR22 & ViT-B/16 & IN‑1K & 77.0 & 78.7 & 0.8M & 79.2  & 1.4M & \textcolor{ForestGreen}{+0.5} & 84.0 &  \\
        \cline{2-13} \\ [-4pt]
        & \multirow{2}{*}{DINOv2~\cite{dinov2}}  & \multirow{2}{*}{TMLR24} & ViT-B/14 & \multirow{2}{*}{LVD-142M} & 81.8  & 83.2 & 0.8M & 84.0 & 1.4M &\textcolor{ForestGreen}{+0.8} & \textcolor{red}{$\times$} & \\
        &  & & ViT-L/14 & & 83.5 & 85.2 & 1.0M & 85.6 & 2.1M & \textcolor{ForestGreen}{+0.4} & -- \\
        \cline{2-13} & \\ [-4pt]
        & Franca~\cite{franca}  & arXiv25 &  ViT-L/14 & IN-21k & 82.2 & 83.8 & 1.0M & 84.3 & 2.1M & \textcolor{ForestGreen}{+0.5} & -- & \\
        \cline{2-13} \\ [-4pt]
        & \multirow{2}{*}{DINOv3~\cite{dinov3}}  & \multirow{2}{*}{arXiv25} & ViT-B/16 & \multirow{2}{*}{LVD-1689M} & 83.0 & 84.0 & 0.8M & 84.4 & 1.4M &\textcolor{ForestGreen}{+0.4} & -- & \\
        & & & ViT-L/16 & & 85.3 & 86.6 & 1.0M & 87.1 & 2.1M & \textcolor{ForestGreen}{+0.5} & -- & \\
        \midrule
        \multirow{3}{*}{\rotatebox{90}{VLM}} & CLIP~\cite{radford2021clip}    & PMLR21 & ViT-L/14 & WIT & 77.2  & 82.3 & 0.8M & 83.4  & 2.1M & \textcolor{ForestGreen}{+1.1} & \textcolor{red}{$\times$} & \\
        & SigLIP~\cite{siglip}  & ICCV23 & ViT-L/16 & WebLI & 83.7  & 85.9 & 1.0M & -- & 2.1M & \textcolor{ForestGreen}{+--} & \textcolor{red}{$\times$} & \\
        & SigLIP2~\cite{siglip2}  & arXiv25 & ViT-L/16 & WebLI & 84.4  & 86.9 & 1.0M & -- & 2.1M & \textcolor{ForestGreen}{+--} & \textcolor{red}{$\times$} & \\
        \midrule
        \multirow{3}{*}{\rotatebox{90}{GEN}} & DiT~\cite{dit}    & ICCV23 & DiT-XL/2 & IN‑1K & -- & 32.7 & 1.2M & 57.0 & 2.5M & \textcolor{ForestGreen}{+24.3} & -- & \\
        & SiT~\cite{sit}    & ECCV24 & DiT-XL/2 & IN‑1K & -- & -- & 1.2M & -- & 2.5M &  -- & -- & \\
        & AIMv2~\cite{aimv2} & CVPR25 & ViT-L/14 & custom$^{*}$ & 80.8 & 84.8 & 1.0M & 85.9 & 2.1M & \textcolor{ForestGreen}{+1.1} & -- & \\
        \bottomrule
    \end{tabular}

==> tab/imagenet_val_masks.tex <==
%------------------------------------------------------------------------------
\begin{figure*}
\scriptsize
\centering
\setlength{\tabcolsep}{1.4pt}
\newcommand{\sz}{.2}
\begin{tabular}{cccccc}

%--- Row 1 ---
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000029_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000091_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000138_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00047373_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000263_overlay.jpg} &
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000446_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00038435_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00048745_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000603_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000654_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000683_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000901_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00000925_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001070_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00047343_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001158_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001167_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001190_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001334_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001392_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001493_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001541_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001546_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001650_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001712_overlay.jpg} \\
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001753_overlay.jpg} &
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001785_overlay.jpg} &
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001793_overlay.jpg} &
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001865_overlay.jpg} &
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001887_overlay.jpg} &
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001890_overlay.jpg} \\
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00001988_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00037971_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00002146_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00002158_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00002167_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00002223_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00002766_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00003091_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00003134_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00003624_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00003701_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00004773_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00005063_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00005178_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00005515_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00005579_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00007490_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00007698_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00013439_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00015295_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00016054_overlay.jpg} &
%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00017809_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00037475_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00018046_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00018286_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00018616_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00018806_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00018833_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00019631_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00022487_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00022718_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00022884_overlay.jpg} \\
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00025557_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00027744_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00033660_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00033890_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00036146_overlay.jpg} &
\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00037120_overlay.jpg} \\


%\includegraphics[width=2.5cm,height=2cm]{fig/imagenet_val_masks/ILSVRC2012_val_00048935_overlay.jpg} &

\end{tabular}
\caption{\emph{Visualization of ImageNet-1k validation masks} created for our localization experiments.}
\label{fig:masks}
\end{figure*}
%------------------------------------------------------------------------------

==> tab/old_imagenet_val_extended_comparisons.tex <==
    \begin{tabular}{c|lcccrrrrrr}
        \toprule
         & \textsc{Method} & \textsc{Pub} & \textsc{Arch} & \textsc{Pre-training} & k-NN  & LP & EP & \textsc{Gain} & EP$^{\star}$ & FT \\
        \midrule
        \multirow{6}{*}{\rotatebox{90}{MIM}} 
        & \multirow{3}{*}{MAE~\cite{mae}}     & \multirow{3}{*}{CVPR22} & ViT-S/16 & \multirow{3}{*}{IN-1K} & 26.7 & 47.4 & 64.6 & \textcolor{ForestGreen}{+17.2} & 65.4 & 80.6$^{\dagger}$ \\
        & &  & ViT-B/16 &  & 46.1 & 67.7 & 75.6 & \textcolor{ForestGreen}{+7.9} & 76.0 & 83.6 \\
        & &  & ViT-L/16 &  & 58.2 & 76.0 & 79.3 & \textcolor{ForestGreen}{+3.3} & & 85.9 \\
        \cline{2-11} \\ [-4pt]
        & BEiTv2~\cite{beitv2}  & arXiv22 & ViT-B/16 & IN‑1K & 74.8 & 79.0  & 81.7 & \textcolor{ForestGreen}{+2.7} & 81.7 & 85.0 \\
        & SimMIM~\cite{simMIM}  & CVPR22 & ViT-B/16 & IN‑1K & 15.1 & 51.5  & 65.1 & \textcolor{ForestGreen}{+13.6} & & 83.8  \\
        & CAPI~\cite{capi}    & TMLR25 & ViT-L/14 & IN‑1K & 76.7  & 81.5  & 83.6 & \textcolor{ForestGreen}{+2.1} & & \textcolor{red}{$\times$} \\
        \midrule
        \multirow{2}{*}{\rotatebox{90}{JEA}} & BYOL~\cite{byol}    & NeurIPS20 & RN-50 & IN‑1K & 64.8  & 74.3 & 75.1 & \textcolor{ForestGreen}{+0.8} & & 77.7  \\
        & DINO~\cite{caron2021emerging}    & ICCV21 & ViT-B/16 & IN‑1K & 76.1  & 77.3 & 77.8 & \textcolor{ForestGreen}{+0.5} & & 82.8  \\
        \midrule
        \multirow{7}{*}{\rotatebox{90}{HYBRID}} & iBOT~\cite{ibot}    & ICLR22 & ViT-B/16 & IN‑1K & 77.0 & 78.7 & 79.2  & \textcolor{ForestGreen}{+0.5} & & 84.0  \\
        \cline{2-11} \\ [-4pt]
        & \multirow{2}{*}{DINOv2~\cite{dinov2}}  & \multirow{2}{*}{TMLR24} & ViT-B/14 & \multirow{2}{*}{LVD-142M} & 81.8  & 83.2 & 84.0  &\textcolor{ForestGreen}{+0.8} & & \textcolor{red}{$\times$} \\
        &  & & ViT-L/14 & & 83.5 & 85.2 & 85.6 & \textcolor{ForestGreen}{+0.4} & & -- \\
        \cline{2-11} \\ [-4pt]
        & Franca~\cite{franca}  & arXiv25 &  ViT-L/14 & IN-21k & 82.2 & 83.8 & 84.3 & \textcolor{ForestGreen}{+0.5} & -- \\
        \cline{2-11} \\ [-4pt]
        & \multirow{2}{*}{DINOv3~\cite{dinov3}}  & \multirow{2}{*}{arXiv25} & ViT-B/16 & \multirow{2}{*}{LVD-1689M} & 83.0 & 84.0 & 84.4 & \textcolor{ForestGreen}{+0.4} & -- \\
        & & & ViT-L/16 & & 85.3 & 86.6 & 87.1 & \textcolor{ForestGreen}{+0.5} & -- \\
        \midrule
        \multirow{3}{*}{\rotatebox{90}{VLM}} & CLIP~\cite{radford2021clip}    & PMLR21 & ViT-L/14 & WIT & 77.2  & 82.3 & 83.4  & \textcolor{ForestGreen}{+1.1} & \textcolor{red}{$\times$} \\
        & SigLIP~\cite{siglip}  & ICCV23 & ViT-L/16 & WebLI & 83.7  & 85.9  & -- & \textcolor{ForestGreen}{+--} & \textcolor{red}{$\times$} \\
        & SigLIP2~\cite{siglip2}  & arXiv25 & ViT-L/16 & WebLI & 84.4  & 86.9  & -- & \textcolor{ForestGreen}{+--} & \textcolor{red}{$\times$} \\
        \midrule
        \multirow{3}{*}{\rotatebox{90}{GEN}} & DiT~\cite{dit}    & ICCV23 & DiT-XL/2 & IN‑1K & -- & 32.7 & 57.0 & \textcolor{ForestGreen}{+24.3} & -- \\
        & SiT~\cite{sit}    & ECCV24 & DiT-XL/2 & IN‑1K & -- & -- & -- &  -- & --\\
        & AIMv2~\cite{aimv2} & CVPR25 & ViT-L/14 & custom$^{*}$ & 80.8 & 84.8 & 85.9 & \textcolor{ForestGreen}{+1.1} & -- \\
        \bottomrule
    \end{tabular}

==> tex/defn.tex <==
% defn.tex — macros (ICLR-safe)

% --- Load tiny deps only if needed (and only in the preamble) ---
\makeatletter
\@ifpackageloaded{xspace}{}{%
  \RequirePackage{xspace}%
}
\@ifpackageloaded{xcolor}{}{%
  \RequirePackage{xcolor}%
}
\makeatother

% ===============================
% Project / method name macros
% ===============================
% Text forms
\DeclareRobustCommand{\our}{efficient probing\xspace}   % “We introduce \our ...”
\DeclareRobustCommand{\Our}{Efficient Probing\xspace}   % Sentence-start variant
\DeclareRobustCommand{\OUR}{\textsc{ep}\xspace}         % Short tag in text “(\OUR)”

% Math-safe form (use inside $...$): $\mOUR_M$
\DeclareRobustCommand{\mOUR}{\mathrm{EP}}

% ===============================
% Common labels & abbreviations
% ===============================
% [CLS] token and friends
\DeclareRobustCommand{\cls}{\texttt{[CLS]}\xspace}      % text usage
\DeclareRobustCommand{\CLS}{\mathrm{[CLS]}}             % math usage

\DeclareRobustCommand{\gap}{\textsc{gap}\xspace}        % Global Average Pooling
% If you prefer exact capitalisation “ViT”, just use \textit{ViT} in prose.
% Using small caps for acronyms is common:
\DeclareRobustCommand{\vit}{\textsc{vit}\xspace}

\DeclareRobustCommand{\vs}{vs.\@\xspace}
\DeclareRobustCommand{\eg}{e.g.\@\xspace}
\DeclareRobustCommand{\ie}{i.e.\@\xspace}

% Names of other models/methods
\DeclareRobustCommand{\vjepa}{V-JEPA\xspace}
\DeclareRobustCommand{\coca}{CoCa\xspace}
\DeclareRobustCommand{\simpool}{SimPool\xspace}
\DeclareRobustCommand{\cait}{CaiT\xspace}
\DeclareRobustCommand{\clip}{CLIP\xspace}
\DeclareRobustCommand{\aim}{AIM\xspace}
\DeclareRobustCommand{\siglip}{SigLIP\xspace}
\DeclareRobustCommand{\abmilp}{AbMILP\xspace}
\DeclareRobustCommand{\cae}{CAE\xspace}
\DeclareRobustCommand{\cbam}{CBAM\xspace}
\DeclareRobustCommand{\delf}{DELF\xspace}
\DeclareRobustCommand{\dolg}{DOLG\xspace}
\DeclareRobustCommand{\mhca}{\textsc{mhca}\xspace}  

% ===============================
% Math helpers
% ===============================
\DeclareRobustCommand{\relu}{\mathrm{ReLU}}
\DeclareRobustCommand{\LN}{\mathrm{LN}}

% Colored text helper (safe wrapper around \textcolor)
\DeclareRobustCommand{\Col}[2]{\textcolor{#1}{#2}}

% ===============================
% TikZ/pgfplots-dependent marks (guarded)
% ===============================
\makeatletter
% Small filled dot; falls back if TikZ not loaded
\@ifpackageloaded{tikz}{%
  \DeclareRobustCommand{\all}{%
    \tikz{\draw[white,fill=black,line width=0.4pt] (0,0) circle (1.2pt);}%
  }%
}{%
  \DeclareRobustCommand{\all}{\mbox{\tiny$\bullet$}}%
}

% Custom plot mark only if pgfplots is present
\@ifpackageloaded{pgfplots}{%
  \pgfdeclareplotmark{customhalfcircle}{%
    % left half
    \fill (-\pgfplotmarksize/1.2,-\pgfplotmarksize/1.2)
      arc (180:360:\pgfplotmarksize/1.2) -- cycle;
    % right half
    \fill (\pgfplotmarksize/1.2,-\pgfplotmarksize/1.2)
      arc (0:180:\pgfplotmarksize/1.2) -- cycle;
  }%
}{}
\makeatother

\definecolor{Learn}{HTML}{1B9E77} % muted green
\newcommand{\learn}[1]{\textbf{\textcolor{Learn}{#1}}}



==> tex/intro-1.tex <==
\section{Introduction}
\label{sec:intro}

Self-supervised learning (SSL) has emerged as a powerful paradigm for learning representations without labeled data, significantly reducing the reliance on costly human annotations. Recent advances in SSL can be broadly categorized into two families: joint-embedding architectures and masked image modeling (MIM).

Joint-embedding architectures learn representations by enforcing similarity between different augmentations of the same image, using contrastive, clustering-based, or redundancy reduction objectives~\cite{caron2021emerging, grill2020bootstrap, bardes2022vicreg}. These methods rely on a global representation, often extracted from a dedicated [CLS] token or through pooling operations over patch tokens. On the other hand, MIM methods~\cite{he2022masked, xie2022simmim, peng2022beitv2} reconstruct masked image regions from their visible counterparts, producing feature representations that retain fine-grained spatial information distributed across patch tokens, rather than concentrating information in the [CLS] token.

To evaluate self-supervised representations, standard protocols include k-NN evaluation, linear probing, and full fine-tuning. While fine-tuning achieves the highest performance, it is computationally expensive. Linear probing is more efficient but relies on the [CLS] token, which, as noted in MIM models, may not be the most discriminative representation. Given that valuable information is spread across patch tokens, an emerging alternative is attentive probing, which selectively aggregates relevant features from patch tokens using attention mechanisms.

Despite its increasing adoption, attentive probing has not been systematically explored. Various works employ different forms of attention-based aggregation, yet no study has rigorously compared their effectiveness or efficiency. In this work, we conduct a comprehensive study on attentive probing, benchmarking multiple existing methods and analyzing the impact of attention on representation quality.

We first establish the significance of attention-based selective aggregation by demonstrating a strong correlation between classification accuracy and spatial localization abilities. Our analysis reveals that, rather than relying on shortcut learning (e.g., exploiting background features like water to classify a fish), models trained with attentive probing effectively attend to foreground objects, improving interpretability and robustness.

Building on these insights, we develop an extensive benchmark that includes both previously introduced attentive probing methods and attentive pooling mechanisms. Our results show that while all attentive methods surpass linear probing, many suffer from over-parameterization and unnecessary complexity. To enable a fair comparison, we introduce a unified framework with a consistent formulation and notation, allowing for a systematic dissection of key components in attentive probing.

Through this framework, we isolate the most essential design elements and propose a new efficient attentive probing method, Efficient Probing (EP). Our approach is a multi-query cross-attention mechanism that eliminates the need for key projections, reduces the number of trainable parameters, and achieves a 10× speedup over conventional multi-head cross-attention, while scaling efficiently with an increasing number of queries.

Furthermore, we discover that the representational power of our learned descriptor allows for significant accuracy gains even when reducing the classifier dimensionality. This enables probing with fewer parameters than standard linear probing, making it a more efficient alternative in both computation and memory usage.

We validate our findings through extensive experiments on ten classification benchmarks and across four MIM frameworks (MAE, SimMIM, BEiTv2, CAPI). Our results consistently demonstrate that Efficient Probing (EP) outperforms both linear probing and existing attentive probing methods, achieving a superior accuracy-to-efficiency trade-off.

Our contributions can be summarized as follows:
\begin{itemize}
    \item We conduct the first systematic study on attentive probing, benchmarking existing methods and analyzing their effectiveness in classification tasks.
\end{itemize}

==> tex/intro-2.tex <==
\section{Introduction}
\label{sec:intro}

%------------------------------------------------------------------------------
\begin{figure}[ht]
    \vspace{-7pt}
    \centering
    \input{plots/mae_vitb_cifar100_colors}
%     \vspace{-15pt}
    \caption{We introduce \emph{\our} (\OUR), a lightweight attention mechanism improving efficiency without compromising performance. We benchmark \emph{attentive probing} and \emph{attentive pooling} methods to evaluate frozen models pretrained with Masked Image Modeling (MIM). \OUR matches or surpasses their performance while improving compute, memory, and parameter efficiency, scaling effectively with the number of learnable queries.
%     Notably, its learned descriptor retains representational power, enabling accuracy gains even with reduced classifier dimensionality (e.g. $D_o = \frac{D_i}{4}$).
    Here: Top-1 classification accuracy \vs number of parameters for different methods on CIFAR-100 with MAE ViT-B. CLS: linear probing; GAP: global average pooling; ViT: default transformer block; $\mOUR_M$: \our with $M$ learnable queries.
    \vspace{-12pt}
    \label{fig:bench-cifar}}
\end{figure}
%------------------------------------------------------------------------------

\emph{Self-supervised learning} (SSL)~\cite{simclr, byol, caron2021emerging, ibot, attmask} has emerged as a powerful paradigm for learning visual representations without labeled data, significantly reducing the reliance on costly human annotations. Recent advances in SSL can be broadly categorized into two families: \emph{joint embedding} architectures~\cite{simclr, byol, caron2021emerging, bardes2021vicreg} and \emph{masked image modeling} (MIM)~\cite{mae, chen2023cae, ibot, attmask, maskfeat, beitv2, i-jepa, capi}.
%
Joint embedding architectures learn representations by enforcing similarity between different augmentations of the same image, using contrastive, clustering-based, or redundancy reduction objectives. They rely on a global representation, a dedicated [CLS] token or pooling of patch tokens. On the other hand, MIM methods reconstruct masked image regions from their visible counterparts. Thus, they obtain  representations that preserve fine-grained spatial information distributed across  tokens, rather than concentrating information in the [CLS].

%To evaluate self-supervised representations, standard protocols include $k$-NN evaluation, linear probing, and full fine-tuning. While fine-tuning achieves the highest performance, it is computationally expensive. Linear probing is more efficient but relies on the [CLS] token, which may not be the most discriminative representation in MIM models~\cite{przewikezlikowski2024beyond}. Given that valuable information is spread across patch tokens, an emerging alternative is \emph{attentive probing}~\cite{autoregressive-image-models, chen2023cae, bardes2024jepa, capi}, which selectively aggregates relevant features from patch tokens using attention mechanisms. This protocol provides a more intuitive framework for evaluating the representations learned by MIM approaches, leading to improved performance.


To evaluate self-supervised pre-training, common protocols include k-NN evaluation, linear probing, and full fine-tuning. While k-NN and linear probing assess representation quality, fine-tuning evaluates pre-training as network initialization for downstream tasks. However, MIM models often lack a discriminative global representation~\cite{przewikezlikowski2024beyond}, making k-NN and linear probing inappropriate. Since valuable information is distributed across patch tokens, \emph{attentive probing}~\cite{autoregressive-image-models, chen2023cae, bardes2024jepa, capi} has emerged as an alternative, using attention mechanisms to selectively aggregate relevant features, leading to improved performance. Despite its growing adoption, attentive probing remains underexplored, with various aggregation methods proposed but no rigorous comparison. This work aims to bridge this gap by systematically studying and analyzing its underlying mechanisms.

% To evaluate self-supervised pre-training, common protocols include k-NN evaluation, linear probing, and full fine-tuning. While k-NN and linear probing assess the quality of learned representations, fine-tuning assesses the effectiveness of pre-training as a network initialization for downstream tasks. However, since MIM models typically lack a discriminative global representation, e.g., [CLS]~\cite{przewikezlikowski2024beyond}, evaluating them with k-NN or simple linear probing offers limited insight into their true representational power. Given that valuable information is distributed across patch tokens, an emerging alternative is \emph{attentive probing}~\cite{autoregressive-image-models, chen2023cae, bardes2024jepa, capi}, which selectively aggregates relevant features from patch tokens using attention mechanisms. This protocol provides a more intuitive framework for evaluating the representations learned by MIM approaches, leading to improved performance.

% Despite its increasing adoption, attentive probing has not been systematically explored. Different forms of attention-based aggregation have been suggested, yet no study has rigorously compared their effectiveness and efficiency. In this work, we attempt to improve our understanding by conducting a comprehensive study and analyzing the underlying mechanisms of attentive probing.

We introduce a framework that encompasses a range of attentive probing methods, including those previously proposed in this context as well as in unrelated tasks.
By analyzing the attention mechanism within this framework, we identify several simplifications that lead to a new, more efficient attentive probing method, \emph{\our} (\OUR). \OUR\ is conceptually simple yet significantly more efficient than existing methods in both parameter count and computational complexity, while achieving near state-of-the-art performance (\autoref{fig:bench-cifar}).
Moreover, it effectively balances the trade-offs between accuracy, model size, and computational cost.
Our analysis and results show that while all attentive methods outperform linear probing, many suffer from \emph{over-parameterization} and \emph{unnecessary complexity}.

A key aspect of existing methods and the proposed \OUR is the use of multiple independent \emph{attention predictors} (\eg heads, queries, or other components).
% , each responsible for a subspace of the output.
We establish a connection between the contribution of each predictor to the classification accuracy and its \emph{localization quality}. Our analysis shows that, rather than resorting to shortcut learning, \eg, leveraging background cues like water to classify a fish, \OUR produces attention maps that effectively focus on foreground objects, enhancing both interpretability and robustness. Furthermore, we observe that more spatially focused attention maps lead to improved performance. Notably, each attention predictor in \OUR specializes in distinct object regions, ensuring complementary feature extraction and a more structured representation.

% We first establish the significance of attention-based selective aggregation by demonstrating a strong correlation between classification accuracy and \emph{spatial localization} abilities. Our analysis reveals that, rather than relying on shortcut learning (e.g., exploiting background features like water to classify a fish), models trained with attentive probing effectively attend to foreground objects, improving interpretability and robustness.

% Building on these insights, we develop an extensive benchmark and evaluate several attentive probing -- or attentive pooling that we cast as probing -- mechanisms. Our results show that while all attentive methods outperform linear probing, many suffer from \emph{over-parameterization} and \emph{unnecessary complexity}. To enable a fair comparison, we introduce a unified framework with consistent formulation, allowing for a systematic dissection of key components of attentive probing.

% Through this framework, we isolate the most essential design elements and propose a new attentive probing method, \emph{\our} (\OUR). Our approach is a multi-query cross-attention mechanism that eliminates the need for query and key projections, reduces the number of trainable parameters, and achieves a 10$\times$ speedup over conventional multi-head cross-attention, while scaling efficiently with an increasing number of queries.

% We further discover that the representational power of our learned descriptor allows for significant accuracy gains even when reducing the classifier dimensionality. This enables probing with fewer parameters than standard linear probing, making it a more efficient alternative in both computation and memory usage.

We validate our findings through extensive experiments on seven classification benchmarks and across three MIM frameworks (MAE~\cite{mae}, SimMIM~\cite{simMIM}, BEiTv2~\cite{beitv2}). Our results consistently demonstrate that our \our outperforms both linear probing and existing attentive probing methods, achieving a superior \emph{accuracy-to-efficiency} trade-off.
In particular, \OUR achieves a 10$\times$ speedup and 1.5$\times$ parameter reduction over the best existing method that relies on conventional multi-head cross-attention.

Our contributions are summarized as follows:
\begin{enumerate}
    \item We conduct the first systematic study on attentive probing, benchmarking existing methods, analyzing their effectiveness in classification tasks.
    %  and \todo{studying how this relates to the quality of attention maps}.
    \item We derive a new probing mechanism, \emph{\our} (\OUR), which is on par with the state-of-the-art, while bringing spectacular gains in compute, memory, and parameter efficiency.
    \item Our analysis provides insights into the importance of spatial localization in attentive probing.
\end{enumerate}

==> tex/method-1.tex <==
\section{Method}
\label{sec:method}

\subsection{Preliminaries}
Let $X \in \real^{D \times N}$ be the \emph{feature matrix} obtained from a \emph{pre-trained} and \emph{frozen} ViT backbone, where $D_i$ is the number of feature channels, and $N=W \times H$ the number of features, one per image patch across the spatial dimension $W \times H$.
Given the \emph{input features} $X$ as input the goal is to generate an \emph{output image-level feature}
$\vy \in \real^{D_o}$ by applying an \textbf{attentive pooling} mechanism.
The output feature is used to train a $C$-way linear classifier with $D_o (C+1)$ parameters.

% Let $\tilde{X} \in \real^{D \times W \times H}$ be the three-dimensional feature tensor obtained from a \emph{pre-trained} and \emph{frozen} ViT backbone, where $D_i$ is the number of feature channels, and $W, H$ denote the spatial width and height, respectively. We flatten the spatial dimensions to obtain a \emph{feature matrix} $X \in \real^{D_i \times N}$, also referred to as \emph{input features}, where $N \defn W \times H$ is the number of spatial locations.
% %
% Given features $X$ as input the goal is to generate an \emph{output image-level feature}
% $\vy \in \real^{D_o}$ by applying an \textbf{attentive pooling} mechanism.
% The output feature is used to train a $C$-way linear classifier with $D_o (C+1)$ parameters.

\subsection{Attentive Pooling}
%
Let $\va_j \in \real^N$ be an $\lone$-normalized vector of attention weights produced by an attention predictor, with $j \in \{1, \ldots, M\}$ and $M$ predictors in total.
Each attention vector, reshaped to $W \times H$, is an attention map indicating the locations at which the $j$-th predictor focuses on.
Let $V \in \real^{D_o \times N}$ be the transformed features,
most commonly obtained via a linear transformation
 by $V=W_V X$, where $W_V \in \real^{D_o \times D_i}$ is a learnable projection matrix.

Assuming the output feature is split into $M$ subvectors
%
\begin{equation}
\vy = \begin{bmatrix} \vy_1 \\ \vdots \\ \vy_M \end{bmatrix} ,
\end{equation}
%
with $\vy_j \in \real^{d^\prime}$, the attentive pooling operation is then given by
%
\begin{equation}
\vy_j = V_j \va_j = W_{V_j} X \va_j
\end{equation}
%
where
\begin{equation}
W_V =  \begin{bmatrix} W_{V_1} \\ \vdots \\ W_{V_M} \end{bmatrix},
V =  \begin{bmatrix} V_1 \\ \vdots \\ V_M \end{bmatrix},
\end{equation}
and $V_j \in \real^{d_o \times N}$, $W_{V_j} \in \real^{d_o \times D}$, $d_o = \frac{D_o}{M}$.
Each attention predictor is responsible for the weighted aggregation of $N$ features into a $d_o$-dimensional subspace of the final representation space. In the following, we explore existing and novel ways for designing these attention predictors.
We focus on the number of additional parameters to be learnt on top of the frozen backbone, and the computational complexity of the pooling operation.

\subsection{Attention Predictors}
%
\paragraph{Multi-Head Cross-Attention (MHCA)}
A standard approach is to perform multi-head cross-attention between the input features and a separate \alert{input vector} $\vu \in \real^D_i$, where each head corresponds to a separate predictor of  attention weights.
%
Linear transformation by $W_K \in \real^{D_a \times D_i}$ and  $W_Q \in \real^{D \times D_i}$ generates the key features $K= W_Q X \in \real^{D_a \times N}$ and the query feature by $\vq = W_Q \vu  \in \real^D_a$.
Attention for head $j$ is given by $\va_j = \softmax(\hat{\va}_j)$ with
%
\begin{equation}
\hat{\va}_j = K_j^\top \vq_j = (W_{K_j}  X)^\top (W_{Q_j} \vu )
\label{equ:mha}
\end{equation}
%
where
%
\begin{equation}
W_K =  \begin{bmatrix} W_{K_1} \\ \vdots \\ W_{K_M} \end{bmatrix},
K =  \begin{bmatrix} K_1 \\ \vdots \\ K_M \end{bmatrix},
\end{equation}
%
and $K_j \in \real^{d_a\times N}$, and $W_{K_j} \in \real^{d_a \times D_a}$,
and equivalently
%
\begin{equation}
  W_Q =  \begin{bmatrix} W_{Q_1} \\ \vdots \\ W_{Q_M} \end{bmatrix},
  \vq =  \begin{bmatrix} \vq_1 \\ \vdots \\ \vq_M \end{bmatrix},
  \end{equation}
%
with $d_a = \frac{D_a}{M}$.

Input features and input vector are projected to $d_a$-dimensional subspaces where attention weights are computed via dot product.
This attention predictor requires $D_a(2D_i+1)$ parameters, and has complexity $\mathcal{O}(ND_a D_i+1)$.
There are several existing methods that fit within this generic framework with little or no differences. These are discussed in Section \ref{sec:var}.

\paragraph{MHCA with a learnable query feature}
%
If we consider $\vu$ to be learnable, then, in \equ{mha} there is no need for the additional parameters of $W_Q$. We can equivalently set the query vector $\vq$ to be learnable, and consequently is subvectors $\vq_j$ too.
% This reduces the number of additional parameters to be learnt and saves from a matrix to vector multiplication in obtaining the query feature.
Removing the query transformation simplifies the architecture, reduces the amount of computations and the number of parameters down to $D_a(D_i+1)$.
Equation \equ{mha} is then rewritten as
\begin{equation}
\hat{\va}_j = X^\top W_{K_j}^\top \vq_j
\end{equation}
where $\vq_j \in \real^d_a$ is learnable, and $W_{K_j}^\top$ maps it to the $D_i$-dimensional space of the input features where attention weights are computed.
%
Therefore, standard MHCA ensures that each query subvector, consequently each attention predictor (head), despite defined in a smaller dimensional space is interacting with the full representation space of the input features.

We consider further simplifying the architecture by removing the key transformation.
Let $W_K$ be fixed to identity matrix and observe how $W_{K_j}$ makes the query only interact with a $\frac{D_i}{M}$-dimensional subspace of the input features.
This is a limitation which we experimental verify to perform poorly.
In the following, we suggest a new way to design new attention predictors that has less parameters, require less compute and overcome this limitation which makes them perform better.
% \bill{While reducing query projections already simplifies the architecture, we explore whether we can entirely remove parameter matrices by learning queries directly in the original feature space, bypassing (unnecessary) transformations.}
%

\paragraph{Transformation-free Cross-Attention with multiple learnable query features}
%
% \bill{needs more details here to understand - polish: In standard multi-head cross-attention, each head operates on a projected subspace of the feature channels via  $W_K$ , ensuring that queries interact with the full input feature representation. However, simply removing  $W_K$  without modification forces query subvectors to attend only to their corresponding feature slices, significantly limiting their expressive capacity. To overcome this, we propose to learn multiple full-dimensional query vectors \( \vq_j \in \mathbb{R}^{D_i} \), allowing direct comparison with the entire input feature matrix  X  without requiring additional projections. This ensures that each query aggregates information from the full feature dimension rather than a restricted subspace, improving both efficiency and expressiveness.}
Instead of using parts of $W_K$ to project query subvectors to the input feature space, we propose to learn multiple query vectors $\vq_j \in \real^D_i$ in the original $D_i$-dimensional space to directly compare with the input features and without any additional processing.
This reduces the number of additional parameters to be learnt and saves from a matrix to matrix multiplication. Note that this variant does not include the standard parameter matrices of attention, and has no other parameters than the learnable query vectors.
Now the attention prediction becomes
\begin{equation}
\hat{\va}_j = X^\top \vq_j,
  \end{equation}
 with $j \in \{1, \ldots, M\}$.
%
This approach requires $D_i M$ parameters for the attention, compared to $D_a(D_i+1)$ for the approach in \equ{mha},
while the amount of required operations drops to $ND_i M$ compared to $ND_a(D_i+1)$.
Typically, $M$ is one to two orders of magnitude smaller than $D_i$ and $D_a$, which are commonly equal to each other, making the proposed approach more efficient in terms of both parameters and operations.


\subsection{Existing variants}
\label{sec:var}
\paragraph{AbMILP}

Attention‐based Multiple Instance Learning Pooling~\cite{rymarczyk2021abmilp}
can be viewed as the simplest instance of our MHCA with a learnable query feature framework, with a single head ($M=1$) and no learnable projection on the input features.
Given $X \in \mathbb{R}^{D_i \times N}$,
it introduces a single learnable query vector $\mathbf{q} \in \mathbb{R}^{D_i}$.
Omitting any key projection matrix $W_{K}$, the ``key” features are effectively just $X$ itself. The attention predictor produces
\[
\hat{\va}_1
\;=\;
X^\top \, \mathbf{q}
\;\;\in\; \mathbb{R}^{N},
\quad
\va_1 = \mathrm{softmax}(\hat{\va}_1).
\]
%That is, each spatial location $j$ has logit $(X^\top\mathbf{q})_j$.
%The attention map $\va_1 \in \mathbb{R}^{N}$ is thus $\ell_1$‐normalized.

For the final aggregation, it also omits any value projection $W_{V_1}$,
so the transformed features $V_1 = X$ directly serve as values.
Hence, the pooled descriptor is
\begin{equation}
\vy_1
\;=\;
V_1 \,\va_1
\;=\;
X\,\va_1
\;\;\in \;\mathbb{R}^{D_i}.
\end{equation}
If needed, one may append a linear mapping $W_{V_1}\in \mathbb{R}^{D_o \times D_i}$
to produce $\vy_1\in \mathbb{R}^{D_o}$, but the simplest version sets $W_{V_1}=I$
and yields $\vy_1 \in \mathbb{R}^{D_i}$.
Overall, AbMILP adds only $D_i$ new parameters for the query $\mathbf{q}$, and has complexity $\mathcal{O}(N\,D_i)$ for each forward pass. While parameter‐efficient, it uses just \emph{one} head, so it may capture fewer spatial patterns than multi‐head variants.

\paragraph{AIM}~\cite{autoregressive-image-models} is also an instance of our MHCA with learnable query feature framework that includes a batch normalization on the input features, followed by learnable projections for the keys and values. Let $\mathrm{BN}(\cdot)$ denote a batch‐norm acting columnwise. AIM first computes
\begin{equation}
    X_{\mathrm{bn}} = \mathrm{BN}(X),
\end{equation}
and then defines two linear mapping matrices $W_{k} \in \mathbb{R}^{D_a \times D_i},$ and $W_{v} \in \mathbb{R}^{D_o \times D_i}$ to produce the key and value features
\[
K = W_{k}\,X_{\mathrm{bn}}
\;\;\in\;\mathbb{R}^{D_a\times N},
\quad
V = W_{v}\,X_{\mathrm{bn}}
\;\;\in\;\mathbb{R}^{D_o\times N}.
\]
In practice, one often sets $D_i = D_a = D_o$.
AIM introduces a single query vector $\mathbf{q}\in\mathbb{R}^{D_a}$,
but splits it into $M$ heads.
Each head $j$ forms attention logits
\[
\hat{\mathbf{a}}_j
\;=\;
(K_j)^\top \mathbf{q}_j
\;\;\in \mathbb{R}^{N},
\quad
\mathbf{a}_j = \softmax(\hat{\mathbf{a}}_j)\;\in \mathbb{R}^{N},
\]
and aggregates
\[
\vy_j
\;=\;
V_j \,\mathbf{a}_j
\;\;\in\mathbb{R}^{d^\prime}.
\]
Finally, AIM concatenates
$\{\mathbf\vy_1 ,\dots,\vy_M \}$
into a single descriptor
$\vy \in\mathbb{R}^{d^\prime M} = \mathbb{R}^{D_o}$. Hence, AIM can exploit multiple heads to attend to different spatial patterns. When $D_a=D_o=D_i$, $W_K,W_V$ each have $D_i^2$ parameters and $\mathbf{q}$ has $D_i$,
leading to about $2\,D_i^2 + D_i$ learnable parameters (plus any BN parameters). The main forward cost comes from key/query and value multiplications, giving $\mathcal{O}(2\,N\,D_i^2)$ \bill{wrong? do we put "2" there?}complexity per pass.

\paragraph{DELF}~\cite{delf} \bill{here not sure how to write it, cause if we write it as MHCA with learnable query, then the K will be simple RELU($W_K$X)}

\paragraph{SimPool}~\cite{psomas2023simpool} can be viewed as an instance of the MHCA framework, with a data-driven query vector derived from the average of the input features, a single head ($M=1$) and a layer normalization on the input features. Specifically, let
\[
X_{\mathrm{ln}} \;=\; \mathrm{LN}(X)
\quad(\text{columnwise LN}),
\]
and define the query as
\[
\mathbf{q}
\;=\;
\Bigl(\tfrac{1}{N}\mathbf{1}^\top X\Bigr)\,W_q
\;\;\in\;\mathbb{R}^{D_a},
\]
where $\frac{1}{N}\mathbf{1}^\top X$ is the global average of $X$ (a single $D_i$‐dim vector),
and $W_q\in\mathbb{R}^{D_i\times D_a}$ is a learnable projection. SimPool then forms keys $K$ by
\[
K \;=\; W_{K}\,X_{\mathrm{ln}}
\;\;\in\;\mathbb{R}^{D_a\times N},
\]
for some $W_K\in \mathbb{R}^{D_a\times D_i}$, and treats $X_{\mathrm{ln}}$ itself as the values.
The single‐head attention logits are
\[
\hat{\mathbf{a}} \;=\; K^\top \mathbf{q}
\;\;\in\;\mathbb{R}^N,
\quad
\mathbf{a} = \mathrm{softmax}(\hat{\mathbf{a}}),
\]
and the final descriptor is
\[
\vy
\;=\;
X_{\mathrm{ln}}\,\mathbf{a}
\;\;\in\;\mathbb{R}^{D_o}.
\]
In practice, one often again sets $D_i = D_k = D_o$, so SimPool introduces about $D_i^2 + D_i$ additional parameters
(\ie, the key matrix $W_K$ of size $D_i \times D_i$ and the query transform $W_q$).
The forward pass primarily costs $\mathcal{O}\bigl(N\,D_i^2\bigr)$
from the multiplication $W_K \, X$.

\paragraph{V-Jepa} \bill{let's include cause it belongs to another family - draft not ready at all...}
V-Jepa also applies a single‐query cross‐attention to the input features
$X \in \mathbb{R}^{D_i\times N}$, followed by a residual + MLP “complete block.”
First, a layer normalization is applied:
\[
X_{\mathrm{ln}}
\;=\;
\mathrm{LN}(X)
\;\in\mathbb{R}^{D_i\times N}.
\]
It defines a single query $\mathbf{q}\in\mathbb{R}^{D}$ (optionally transformed by a matrix $W_q\in\mathbb{R}^{D\times D}$),
and two learnable matrices
\[
W_{K}\in \mathbb{R}^{D_i\times D},
\quad
W_{V}\in \mathbb{R}^{D_i\times D},
\]
that yield keys/values:
\[
K = W_{K}^\top\,X_{\mathrm{ln}}
\;\;\in\mathbb{R}^{D\times N},
\quad
V = W_{V}^\top\,X_{\mathrm{ln}}
\;\;\in\mathbb{R}^{D\times N}.
\]
Then V-Jepa computes attention logits
\[
\hat{\mathbf{a}}
=
\bigl(\mathbf{q}\,W_q\bigr)\;K^\top
\quad,
\quad
\mathbf{a} = \mathrm{softmax}(\hat{\mathbf{a}})\;\in\mathbb{R}^N,
\]
and aggregates
\[
\mathbf{x}_\mathrm{attn}
=
\mathbf{a}\;V^\top
\;\in\mathbb{R}^D.
\]
A linear projection $W_{\mathrm{proj}}\in\mathbb{R}^{D\times D}$ is then applied and
\emph{residually} added to $\mathbf{q}$, followed by another layer norm and an MLP block
(\eg, $\mathrm{GELU}$ + two linear layers, again with a residual).
Hence, each forward pass updates $\mathbf{q}$ with cross‐attention to $X$, plus an MLP,
and optionally repeats this “complete block” multiple times if $\textit{depth}>1$.
In the end, $\mathbf{q}\in\mathbb{R}^D$ serves as the pooled image descriptor.

==> tex/method-2.tex <==
\section{Method}
\label{sec:method}

\subsection{Preliminaries}

Let $X \in \real^{D_i \times N}$ be the \emph{feature matrix} obtained from a \emph{pre-trained} and \emph{frozen} ViT backbone, where $D_i$ is the number of feature channels  and $N = W \times H$ the number of features, one per image patch across the spatial dimensions $W \times H$. Given the \emph{input features} $X$, the goal is to generate an \emph{output image-level feature} $\vy \in \real^{D_o}$ by applying an \textbf{attentive pooling} mechanism. The output feature is used to train a $C$-way linear classifier with $D_o (C+1)$ parameters.

%------------------------------------------------------------------------------

\subsection{Attentive Pooling}
\label{sec:att-pool}

We consider $M$ \emph{attention predictors}, to be discussed in \autoref{sec:att-pred}. For each predictor $j \in \{1, \ldots, M\}$, let $\va_j \in \real^N$ be the $\lone$-normalized \emph{attention vector} it generates. Each vector, reshaped to $W \times H$, is an attention map indicating the locations on which the predictor focuses. Let $V \in \real^{D_o \times N}$ be the \emph{transformed features}, commonly obtained by a linear transformation $V=W_V X$, where $W_V \in \real^{D_o \times D_i}$ is a learnable \emph{projection matrix}.

Let the output feature $\vy$, transformed features $V$ and projection matrix $W_V$ be split into $M$ subvectors / submatrices according to
%
\begin{equation}
	\vy = \begin{bmatrix} \vy_1 \\ \vdots \\ \vy_M \end{bmatrix},
	V =  \begin{bmatrix} V_1 \\ \vdots \\ V_M \end{bmatrix},
	W_V =  \begin{bmatrix} W_{V_1} \\ \vdots \\ W_{V_M} \end{bmatrix},
\end{equation}
%
with $\vy_j \in \real^{d_o}$, $V_j \in \real^{d_o \times N}$, $W_{V_j} \in \real^{d_o \times D}$ and $d_o = \frac{D_o}{M}$.

The attentive pooling operation is then given by
%
\begin{equation}
	\vy_j = V_j \va_j = W_{V_j} X \va_j.
	\label{equ:att-pool}
\end{equation}
%
Each attention predictor is responsible for the weighted pooling of $N$ features into a $d_o$-dimensional subspace of the final representation space. In the following, we explore existing and novel ways for designing these attention predictors. We focus on the number of additional parameters to be learnt on top of the frozen backbone and the computational complexity of the pooling operation.

%------------------------------------------------------------------------------

\subsection{Attention Predictors}
\label{sec:att-pred}

\paragraph{Multi-Head Cross-Attention (MHCA)}

A standard approach is to perform multi-head cross-attention between the input features and an \emph{\alert{input vector}} $\vu \in \real^{D_i}$, where each head corresponds to a separate attention predictor. The \emph{query feature} $\vq \in \real^{D_a}$ and \emph{key features} $K \in \real^{D_a \times N}$ are obtained by linear transformations $\vq = W_Q \vu$, $K = W_K X$ with projection matrices $W_Q, W_K \in \real^{D_a \times D_i}$.

Let the query feature $\vq$ and associated projection matrix $W_Q$ be split into $M$ subvectors / submatrices according to
%
\begin{equation}
	\vq =  \begin{bmatrix} \vq_1 \\ \vdots \\ \vq_M \end{bmatrix},
	W_Q =  \begin{bmatrix} W_{Q_1} \\ \vdots \\ W_{Q_M} \end{bmatrix},
\end{equation}
%
with $\vq_j = W_{Q_j} \vu \in \real^{d_a}$, $W_{Q_j} \in \real^{d_a \times D_i}$ and $d_a = \frac{D_a}{M}$. Similarly, let the key features $K$ and associated projection matrix $W_K$ be split according to
%
\begin{equation}
	K =  \begin{bmatrix} K_1 \\ \vdots \\ K_M \end{bmatrix},
	W_K =  \begin{bmatrix} W_{K_1} \\ \vdots \\ W_{K_M} \end{bmatrix},
\end{equation}
%
with $K_j = W_{K_j} X \in \real^{d_a \times N}$ and $W_{K_j} \in \real^{d_a \times D_i}$.

The attention vector for head $j$ is then given by $\va_j = \softmax(\hat{\va}_j)$ with
%
\begin{equation}
\hat{\va}_j = K_j^\top \vq_j = (W_{K_j} X)^\top (W_{Q_j} \vu).
\label{equ:mha}
\end{equation}

That is, the input features $X$ and \alert{input vector} $\vu$ are projected to $d_a$-dimensional subspaces where attention subvectors are computed via dot product followed by softmax normalization over patches. This attention predictor requires $D_a(2D_i+1)$ parameters and has complexity $\mathcal{O}(ND_a D_i+1)$. As discussed in \autoref{sec:var}, there are several existing methods that fit within this generic framework with little or no differences.

%------------------------------------------------------------------------------

\paragraph{MHCA with a learnable query feature}

If we consider \alert{input vector} $\vu$ to be learnable, then there is no need for the projection matrix $W_Q$ in \equ{mha}. Instead, we can set the query feature $\vq$ to be learnable, thus absorbing $W_Q$ and $\vu$:
%
\begin{equation}
	\hat{\va}_j = (W_{K_j} X)^\top \vq_j = X^\top W_{K_j}^\top \vq_j
\label{equ:mha-lrn-q}
\end{equation}
%
where $\vq_j \in \real^{d_a}$ is learnable.

We observe that $W_{K_j}^\top$ maps $\vq_j$ to the $D_i$-dimensional space of input features to compute the attention vector. Thus, standard MHCA ensures that each query subvector
% consequently each attention predictor (head),
is interacting with the full representation space of the input features, despite being defined in a smaller dimensional space. Using a learnable query feature directly simplifies the architecture, reduces the amount of computations \alert{(to what?)} and the number of parameters to $D_a (D_i+1)$.

We consider further simplifying the architecture by removing the key transformation. By letting $W_K$ be fixed to the identity matrix, \equ{mha-lrn-q} becomes
%
\begin{equation}
	\hat{\va}_j = X_j^\top \vq_j
\label{equ:mha-lrn-q-id}
\end{equation}
%
where the feature matrix $X$ is split into $M$ submatrices according to
%
\begin{equation}
	X = \begin{bmatrix} X_1 \\ \vdots \\ X_M \end{bmatrix},
\end{equation}
%
with $X_j \in \real^{d_i \times N}$ and $d_i = \frac{D_i}{M}$. We thus observe that the query feature only interacts  with a $d_i$-dimensional subspace of the input features. This is a limitation that we experimentally verify to perform poorly. In the following, we suggest a new way to design attention predictors that have less parameters, require less compute and overcome this limitation, making them perform better.

%------------------------------------------------------------------------------

\paragraph{Transformation-free Cross-Attention with multiple learnable query features}


Instead of using the key submatrices $W_{K_j}$ to project the query subvectors $\vq_j$ to the $D_i$-dimensional input feature space, we propose to learn multiple \alert{input vectors} $\vu_j \in \real^{D_i}$ in that space directly.  Thus, $\vu_j$ absorbs $W_{K_j}$ and $\vq_j$ and attention prediction becomes
%
\begin{equation}
	\hat{\va}_j = X^\top \vu_j
	\label{equ:ours}
\end{equation}
%
for $j \in \{1, \ldots, M\}$. As a result, there are no projection matrices and there are no parameters other than the learnable \alert{input vectors} $\vu_j$.

This choice reduces the number of additional parameters to be learnt and saves from one more matrix-vector multiplication. In particular, it requires $D_i M$ parameters for the attention compared to $D_a(D_i+1)$ for \equ{mha}, while the number of operations drops to $ND_i M$ compared to $ND_a(D_i+1)$. Typically, $M$ is one to two orders of magnitude smaller than $D_i$ and $D_a$, which are commonly equal to each other, making the proposed approach more efficient in terms of both parameters and operations.

%------------------------------------------------------------------------------

\subsection{Existing variants}
\label{sec:var}
We analyze several existing methods as instances of the presented framework and further examine common variants, considering their relationship to the framework despite slight deviations.

\paragraph{AbMILP}
Attention‐based Multiple Instance Learning Pooling~\cite{rymarczyk2021abmilp}
is the simplest variant.
It fixes $W_V$ to identity and is equivalent to MHCA with a learnable query feature framework in \equ{mha-lrn-q}, with a single head ($M=1$).
It can also be seen as a special case of our proposed method  in \equ{ours} with one \alert{learnable query}, \ie $M=1$.
AbMILP requires only $D_i$ parameters and computes attention with a single matrix to vector multiplication. but its performance is limited by the single head/query.
% AbMILP adds only $D_i$ new parameters, and has complexity $\mathcal{O}(N\,D_i)$, but is limited by the single head/query.

% can be viewed as the simplest instance of our MHCA with a learnable query feature framework, with a single head ($M=1$) and no learnable projection on the input features.
% Given $X \in \mathbb{R}^{D_i \times N}$,
% it introduces a single learnable query vector $\mathbf{q} \in \mathbb{R}^{D_i}$.
% Omitting any key projection matrix $W_{K}$, the ``key” features are effectively just $X$ itself. The attention predictor produces
% \[
% \hat{\va}_1
% \;=\;
% X^\top \, \mathbf{q}
% \;\;\in\; \mathbb{R}^{N},
% \quad
% \va_1 = \mathrm{softmax}(\hat{\va}_1).
% \]
% %That is, each spatial location $j$ has logit $(X^\top\mathbf{q})_j$.
% %The attention map $\va_1 \in \mathbb{R}^{N}$ is thus $\ell_1$‐normalized.

% For the final aggregation, it also omits any value projection $W_{V_1}$,
% so the transformed features $V_1 = X$ directly serve as values.
% Hence, the pooled descriptor is
% \begin{equation}
% \vy_1
% \;=\;
% V_1 \,\va_1
% \;=\;
% X\,\va_1
% \;\;\in \;\mathbb{R}^{D_i}.
% \end{equation}
% If needed, one may append a linear mapping $W_{V_1}\in \mathbb{R}^{D_o \times D_i}$
% to produce $\vy_1\in \mathbb{R}^{D_o}$, but the simplest version sets $W_{V_1}=I$
% and yields $\vy_1 \in \mathbb{R}^{D_i}$.
% Overall, AbMILP adds only $D_i$ new parameters for the query $\mathbf{q}$, and has complexity $\mathcal{O}(N\,D_i)$ for each forward pass. While parameter‐efficient, it uses just \emph{one} head, so it may capture fewer spatial patterns than multi‐head variants.

%------------------------------------------------------------------------------

\paragraph{AIM}~\cite{autoregressive-image-models} is an instance of the MHCA with a learnable query feature framework.
It deviates from the generic framework by applying a batch normalization on the input features.
It fully follows \equ{att-pool} and \equ{mha-lrn-q} with $M$ heads, $D_a = D_i = D_o$, but replaces $X$ by $\mathrm{BN}(X)$ to perform all steps.
Batch normalization introduces additional parameters and a slight computational overhead compared to the default variant of the framework.

% that includes a batch normalization on the input features, followed by learnable projections for the keys and values. Let $\mathrm{BN}(\cdot)$ denote a batch‐norm acting columnwise. AIM first computes
% \begin{equation}
%     X_{\mathrm{bn}} = \mathrm{BN}(X),
% \end{equation}
% and then defines two linear mapping matrices $W_{k} \in \mathbb{R}^{D_a \times D_i},$ and $W_{v} \in \mathbb{R}^{D_o \times D_i}$ to produce the key and value features
% \[
% K = W_{k}\,X_{\mathrm{bn}}
% \;\;\in\;\mathbb{R}^{D_a\times N},
% \quad
% V = W_{v}\,X_{\mathrm{bn}}
% \;\;\in\;\mathbb{R}^{D_o\times N}.
% \]
% In practice, one often sets $D_i = D_a = D_o$.
% AIM introduces a single query vector $\mathbf{q}\in\mathbb{R}^{D_a}$,
% but splits it into $M$ heads.
% Each head $j$ forms attention logits
% \[
% \hat{\mathbf{a}}_j
% \;=\;
% (K_j)^\top \mathbf{q}_j
% \;\;\in \mathbb{R}^{N},
% \quad
% \mathbf{a}_j = \softmax(\hat{\mathbf{a}}_j)\;\in \mathbb{R}^{N},
% \]
% and aggregates
% \[
% \vy_j
% \;=\;
% V_j \,\mathbf{a}_j
% \;\;\in\mathbb{R}^{d^\prime}.
% \]
% Finally, AIM concatenates
% $\{\mathbf\vy_1 ,\dots,\vy_M \}$
% into a single descriptor
% $\vy \in\mathbb{R}^{d^\prime M} = \mathbb{R}^{D_o}$. Hence, AIM can exploit multiple heads to attend to different spatial patterns. When $D_a=D_o=D_i$, $W_K,W_V$ each have $D_i^2$ parameters and $\mathbf{q}$ has $D_i$,
% leading to about $2\,D_i^2 + D_i$ learnable parameters (plus any BN parameters). The main forward cost comes from key/query and value multiplications, giving $\mathcal{O}(2\,N\,D_i^2)$ \bill{wrong? do we put "2" there?}complexity per pass.

%------------------------------------------------------------------------------

\paragraph{DELF}~\cite{delf} Despite not introduced in the context of attentive pooling for SSL we establish an useful relation. DELF feeds each of the $N$ input features to an two-layer MLP whose output is a scalar attention value in $[0,1]$.
It can be viewed as an instance of the MHCA with a learnable query feature framework and $M=1$ with the following two modifications. A non-linearity is introduced in equation \equ{mha-lrn-q} by $\hat{\va} = \relu(W_K X)^\top \vq $, where subscript $j$ is skipped due to $M=1$, and softmax is replaced by the element-wise softplus function $\va = \softplus(\hat{\va})$.
It does not introduce extra parameters and has the same complexity as the default variant of the framework.



%------------------------------------------------------------------------------

\paragraph{SimPool}~\cite{psomas2023simpool}
can be viewed as an instance of the MHCA framework with a single head ($M=1$) but has a data-dependent query vector, $W_V$ fixed to identity, and a layer normalization on the input features.
Specifically average of the input features generates  query $\vq = \frac{1}{N} X^\top \one $ and
 $X$ is replaced by $\mathrm{LN}(X)$ to perform all other steps.
Compared to the default variant of the framework SiPool saves $D_i$ parameters and has the same complexity.

% can be viewed as an instance of the MHCA framework, with a data-driven query vector derived from the average of the input features, a single head ($M=1$) and a layer normalization on the input features. Specifically, let
% \[
% X_{\mathrm{ln}} \;=\; \mathrm{LN}(X)
% \quad(\text{columnwise LN}),
% \]
% and define the query as
% \[
% \mathbf{q}
% \;=\;
% \Bigl(\tfrac{1}{N}\mathbf{1}^\top X\Bigr)\,W_q
% \;\;\in\;\mathbb{R}^{D_a},
% \]
% where $\frac{1}{N}\mathbf{1}^\top X$ is the global average of $X$ (a single $D_i$‐dim vector),
% and $W_q\in\mathbb{R}^{D_i\times D_a}$ is a learnable projection. SimPool then forms keys $K$ by
% \[
% K \;=\; W_{K}\,X_{\mathrm{ln}}
% \;\;\in\;\mathbb{R}^{D_a\times N},
% \]
% for some $W_K\in \mathbb{R}^{D_a\times D_i}$, and treats $X_{\mathrm{ln}}$ itself as the values.
% The single‐head attention logits are
% \[
% \hat{\mathbf{a}} \;=\; K^\top \mathbf{q}
% \;\;\in\;\mathbb{R}^N,
% \quad
% \mathbf{a} = \mathrm{softmax}(\hat{\mathbf{a}}),
% \]
% and the final descriptor is
% \[
% \vy
% \;=\;
% X_{\mathrm{ln}}\,\mathbf{a}
% \;\;\in\;\mathbb{R}^{D_o}.
% \]
% In practice, one often again sets $D_i = D_k = D_o$, so SimPool introduces about $D_i^2 + D_i$ additional parameters
% (\ie, the key matrix $W_K$ of size $D_i \times D_i$ and the query transform $W_q$).
% The forward pass primarily costs $\mathcal{O}\bigl(N\,D_i^2\bigr)$
% from the multiplication $W_K \, X$.

%------------------------------------------------------------------------------

\paragraph{V-Jepa} has its first part identical to the MHCA framework but applies layer normalization on the input features like SimPool. The second part is an MLP with residual connections making the overall process equivalent to a transformer block.
\alert{Params and complexity?}


% V-Jepa also applies a single‐query cross‐attention to the input features
% $X \in \mathbb{R}^{D_i\times N}$, followed by a residual + MLP “complete block.”
% First, a layer normalization is applied:
% \[
% X_{\mathrm{ln}}
% \;=\;
% \mathrm{LN}(X)
% \;\in\mathbb{R}^{D_i\times N}.
% \]
% It defines a single query $\mathbf{q}\in\mathbb{R}^{D}$ (optionally transformed by a matrix $W_q\in\mathbb{R}^{D\times D}$),
% and two learnable matrices
% \[
% W_{K}\in \mathbb{R}^{D_i\times D},
% \quad
% W_{V}\in \mathbb{R}^{D_i\times D},
% \]
% that yield keys/values:
% \[
% K = W_{K}^\top\,X_{\mathrm{ln}}
% \;\;\in\mathbb{R}^{D\times N},
% \quad
% V = W_{V}^\top\,X_{\mathrm{ln}}
% \;\;\in\mathbb{R}^{D\times N}.
% \]
% Then V-Jepa computes attention logits
% \[
% \hat{\mathbf{a}}
% =
% \bigl(\mathbf{q}\,W_q\bigr)\;K^\top
% \quad,
% \quad
% \mathbf{a} = \mathrm{softmax}(\hat{\mathbf{a}})\;\in\mathbb{R}^N,
% \]
% and aggregates
% \[
% \mathbf{x}_\mathrm{attn}
% =
% \mathbf{a}\;V^\top
% \;\in\mathbb{R}^D.
% \]
% A linear projection $W_{\mathrm{proj}}\in\mathbb{R}^{D\times D}$ is then applied and
% \emph{residually} added to $\mathbf{q}$, followed by another layer norm and an MLP block
% (\eg, $\mathrm{GELU}$ + two linear layers, again with a residual).
% Hence, each forward pass updates $\mathbf{q}$ with cross‐attention to $X$, plus an MLP,
% and optionally repeats this “complete block” multiple times if $\textit{depth}>1$.
% In the end, $\mathbf{q}\in\mathbb{R}^D$ serves as the pooled image descriptor.


==> tex/plots-minimal.tex <==
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}
\usepgfplotslibrary{fillbetween}
\newcommand{\kilo}[1]{\thisrow{#1}/1000}


==> tex/related-1.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Evaluation protocols in SSL}

Self-supervised learning (SSL) has revolutionized visual representation learning, offering alternatives to supervised training. Its is typically evaluated via (i) \emph{k-NN evaluation} on frozen features, (ii) \emph{linear probing} with a shallow classifier on a frozen encoder, and (iii) \emph{fine-tuning}, where the entire model is updated, often performing best but at a high computational cost.

Joint embedding architectures (JEA) and masked image modeling (MIM) are two dominant SSL paradigms. JEA methods such as DINO~\cite{caron2021emerging} and SimCLR~\cite{chen2020simple} learn representations by contrasting or clustering different augmentations, leading to strong global representations encoded within a \cls token or a pooled feature. In contrast, MIM methods such as MAE~\cite{mae}, SimMIM~\cite{simMIM}, and BEiT-v2~\cite{beitv2} reconstruct masked image patches, resulting in highly localized feature representations distributed across patch tokens.

This global \vs local distinction between the two paradigms impacts evaluation strategies. Linear probing, relying on the \cls token, serves as an effective evaluation method for JEA~\cite{caron2021emerging} but performs poorly on MIM~\cite{mae}, where discriminative information is spread across patch tokens~\cite{przewikezlikowski2024beyond}. As a result, fine-tuning remains the preferred evaluation strategy for MIM~\cite{mae, simMIM}, despite its higher computational cost. 

Given this limitation, recent work explores \emph{attentive probing}~\cite{autoregressive-image-models, chen2023cae, v-jepa, capi}, which selectively aggregates patch tokens using attention to construct a more informative representation. Although works like AIM~\cite{autoregressive-image-models}, CAE~\cite{chen2023cae}, and V-Jepa~\cite{v-jepa} employ attention-based poolings for probing, no unified evaluation exists. Our work not only bridges this gap by presenting a comprehensive benchmark of attentive probing, but also introduces a novel attentive pooling mechanism achieving strong accuracy-to-efficiency trade-off.

\paragraph{Pooling in vision models}

Pooling is a fundamental operation in visual representation learning, reducing spatial resolution while preserving critical semantic information. In convolutional neural networks (CNNs), pooling is traditionally achieved through fixed operations such as global average pooling (\gap)~\cite{nin, resnet} for classification or regional pooling for detection~\cite{frcnn}. In vision transformers (ViTs)~\cite{vit}, the self-attention mechanism has largely replaced explicit pooling operations, implicitly aggregating spatial information into a single \cls token, effectively serving as a form of global pooling.

Recent works propose explicit attention-based pooling mechanisms that significantly enhance representational capabilities. \simpool~\cite{psomas2023simpool} offers an attention-driven alternative to global average pooling, effectively integrated into both convolutional networks and vision transformers during supervised and self-supervised training. Vision-language models such as \clip~\cite{radford2021clip} and \siglip~\cite{timm} employ attentive pooling for cross-modal feature aggregation, while \coca~\cite{yu2022coca} implicitly utilizes attentive pooling via cross-attention layers between text and visual embeddings. \vjepa~\cite{v-jepa} applies cross-attention pooling in attentive probing to identify informative features from pretrained models. For image retrieval, \delf~\cite{delf} and \dolg~\cite{yang2021dolg} leverage spatial attention to highlight salient keypoints, improving accuracy. \cait~\cite{cait} enhances classification by refining class-token attention, whereas \abmilp~\cite{rymarczyk2021abmilp} introduces single-query attentive pooling for multiple-instance learning. \cbam~\cite{woo2018cbam} sequentially integrates channel and spatial attention to recalibrate convolutional feature maps.

% \todo{In this work, we cast over a dozen existing attentive pooling mechanisms as attentive probing strategies, integrating them into a unified benchmarking framework. Through extensive analysis, we inspect and compare their effectiveness, revealing that while all attentive methods outperform linear probing, many suffer from unnecessary complexity and over-parameterization.}
